Analysis of A Splitting Approach for the Parallel Solution of Linear Systems on GPU Cards

We discuss an approach for solving sparse or dense banded linear systems ${\bf A} {\bf x} = {\bf b}$ on a Graphics Processing Unit (GPU) card. The matrix ${\bf A} \in {\mathbb{R}}^{N \times N}$ is possibly nonsymmetric and moderately large; i.e., $10000 \leq N \leq 500000$. The ${\it split\ and\ parallelize}$ (${\tt SaP}$) approach seeks to partition the matrix ${\bf A}$ into diagonal sub-blocks ${\bf A}_i$, $i=1,\ldots,P$, which are independently factored in parallel. The solution may choose to consider or to ignore the matrices that couple the diagonal sub-blocks ${\bf A}_i$. This approach, along with the Krylov subspace-based iterative method that it preconditions, are implemented in a solver called ${\tt SaP::GPU}$, which is compared in terms of efficiency with three commonly used sparse direct solvers: ${\tt PARDISO}$, ${\tt SuperLU}$, and ${\tt MUMPS}$. ${\tt SaP::GPU}$, which runs entirely on the GPU except several stages involved in preliminary row-column permutations, is robust and compares well in terms of efficiency with the aforementioned direct solvers. In a comparison against Intel's ${\tt MKL}$, ${\tt SaP::GPU}$ also fares well when used to solve dense banded systems that are close to being diagonally dominant. ${\tt SaP::GPU}$ is publicly available and distributed as open source under a permissive BSD3 license.

==> sweepK4DvsCdense.tex <==



The results reported in Table \ref{t:sweepK4DvsCdense} answer the following question: how does $K$ influence the performance of the coupled and uncoupled strategies? Somewhat counterintuitive, when $K$ is large the decoupled strategy performs much better than the coupled counterpart. The explanation is in values listed in the second and third columns. For small $K$, the factorization and spike computation is inexpensive. Although the coupled version is slower in this stage, it wins in the iterative phase owing fast convergence. This fast convergence carries to large values of $K$, yet the pre-processing part ends up dominating and dictating the overall performance of the linear solver.


\pgfplotstableset{
	columns={K,T-PreP-D,T-PreP-C,nItrs-D,nItrs-C,T-Kry-D,T-Kry-C,T-Total-D,T-Total-C,SpeedUp},
	columns/K/.style={
		column name=$K$,
		int detect},
	columns/T-PreP-D/.style={
		dec sep align,
		column name=$D_{pre}$,
		fixed,
		precision=1},
	columns/T-PreP-C/.style={
		dec sep align,
		column name=$C_{pre}$,
		fixed,
		precision=1},
	columns/nItrs-D/.style={
		column name=${D}_{it}$,
		fixed,
		precision=2},
	columns/nItrs-C/.style={
		column name=${C}_{it}$,
		fixed,
		precision=2},
	columns/T-Kry-D/.style={
		dec sep align,
		column name=$D_{Kry}$,
		fixed,
		precision=1},
	columns/T-Kry-C/.style={
		dec sep align,
		column name=$C_{Kry}$,
		fixed,
		precision=1},
	columns/T-Total-D/.style={
		dec sep align,
		column name=$D_{Tot}$,
		fixed,
		precision=1},
	columns/T-Total-C/.style={
		dec sep align,
		column name=$C_{Tot}$,
		fixed,
		precision=1},
	columns/SpeedUp/.style={
		dec sep align,
		column name=\textsc{SpdUp},
		fixed,
		precision=2},
	every head row/.style={
		before row=\toprule,after row=\midrule},
	every last row/.style={
		after row=\bottomrule}}

\begin{table} [ht]
	\label{t:sweepK4DvsCdense}
	\footnotesize
	\centering
	\pgfplotstabletypesetfile{Data/sweepK4DvsCdense.txt}
	\caption{Performance comparison over a spectrum of half bandwidths $K$ for coupled (C) vs. decoupled (D) strategies in {\SpikeHyb}. Problem parameters: $N= \SI{200000}{}$, $P=50$, $d=1$. The meaning of the symbols used is as specified in Table \ref{t:sweepP4DvsCdense}.} 
\end{table}


